Spectroscopic Studies of Type Ia Supernovae Using LSTM Neural Networks

We present a data-driven method based on long short-term memory (LSTM) neural networks to analyze spectral time series of Type Ia supernovae (SNe Ia). The dataset includes 3091 spectra from 361 individual SNe Ia. The method allows for accurate reconstruction of the spectral sequence of an SN Ia based on a single observed spectrum around maximum light. The precision of the spectral reconstruction increases with more spectral time coverages, but the significant benefit of multiple epoch data at around optical maximum is only evident for observations separated by more than a week. The method shows great power in extracting the spectral information of SNe Ia, and suggests that the most critical information of an SN Ia can be derived from a single spectrum around the optical maximum. The algorithm we have developed is important for the planning of spectroscopic follow-up observations of future SN surveys with the LSST/Rubin and the WFIRST/Roman telescopes.

==> Full-Table1.tex <==
\begin{table}
\begin{tabular}{cccccccccc}
SN name & SN subtype & Redshift & Number of spectra & First epoch & Last epoch & Spectrum source & Redshift reference & MJD_max reference & Photometry reference \\
SN2012fr & Ia-norm & 0.005457 & 74 & -13.99 & +30.45 & WISeREP & 1 & 2 & 2 \\
SN2005cf & Ia-norm & 0.006461 & 73 & -12.40 & +29.29 & WISeREP,Kaepora,VLT & 1 & 3 & 4 \\
SN2011fe & Ia-norm & 0.000804 & 68 & -14.82 & +27.51 & WISeREP,Kaepora & 1 & 5 & 6,7 \\
SN2002bo & Ia-norm & 0.004240 & 44 & -13.58 & +29.36 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2006X & Ia-norm & 0.005240 & 40 & -10.68 & +32.07 & WISeREP,Kaepora,VLT & 1 & 3 & 9 \\
SN1994D & Ia-norm & 0.002058 & 38 & -12.47 & +29.44 & Kaepora & 1 & 3 & 10,11 \\
SN2007le & Ia-norm & 0.006721 & 36 & -10.63 & +23.33 & WISeREP,Kaepora & 1 & 3 & 9 \\
SN2003du & Ia-norm & 0.006384 & 35 & -12.70 & +32.98 & Kaepora & 1 & 3 & 12 \\
SN2004dt & Ia-norm & 0.019730 & 32 & -9.44 & +32.72 & WISeREP,Kaepora,VLT & 1 & 3 & 8 \\
SN2003cg & Ia-norm & 0.004130 & 32 & -7.48 & +26.67 & Kaepora & 1 & 3 & 8 \\
SN2001V & Ia-norm & 0.015018 & 27 & -13.20 & +27.97 & WISeREP,Kaepora & 1 & 3 & 13 \\
SN2007af & Ia-norm & 0.005464 & 27 & -5.60 & +32.07 & WISeREP,Kaepora & 1 & 3 & 9 \\
SN2002er & Ia-norm & 0.008569 & 26 & -9.94 & +32.66 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2007co & Ia-norm & 0.026962 & 25 & -5.11 & +30.81 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1999by & Ia-91bg & 0.002128 & 25 & -6.19 & +32.89 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2013dy & Ia-norm & 0.003890 & 24 & -13.28 & +26.52 & WISeREP,Kaepora & 1 & 14 & 6 \\
SN2005hk & Iax & 0.012993 & 24 & -9.29 & +27.17 & WISeREP,Kaepora,VLT & 1 & 3 & 6 \\
SN1999ac & Ia-norm & 0.009500 & 23 & -14.36 & +32.64 & WISeREP,Kaepora & 1 & 3 & 8 \\
SNF20080514-002 & Ia-norm & 0.022095 & 23 & -6.56 & +27.69 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1999dq & Ia-99aa & 0.014327 & 21 & -10.37 & +28.91 & Kaepora & 1 & 3 & 8 \\
SN2001ep & Ia-norm & 0.013129 & 21 & -7.02 & +31.46 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2002dj & Ia-norm & 0.009393 & 21 & -11.39 & +30.12 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1999aa & Ia-99aa & 0.014443 & 20 & -10.98 & +29.30 & WISeREP,Kaepora & 1 & 3 & 15 \\
SN2005am & Ia-norm & 0.007899 & 20 & -2.98 & +31.62 & WISeREP,Kaepora & 1 & 3 & 9 \\
SN2003fa & Ia-99aa & 0.040388 & 20 & -10.36 & +20.36 & Kaepora & 1 & 3 & 8 \\
SN1998bu & Ia-norm & 0.002992 & 20 & -4.55 & +32.36 & WISeREP,Kaepora & 1 & 3 & 15 \\
SN2011iv & Ia-norm & 0.006500 & 20 & -0.94 & +18.85 & WISeREP,VLT & 1 & 16 & - \\
LSQ12gdj & Ia-91T & 0.030000 & 20 & -9.00 & +29.83 & WISeREP & 17 & 18 & 19 \\
SN2006lf & Ia-norm & 0.013206 & 19 & -8.38 & +24.87 & WISeREP,Kaepora & 1 & 3 & 13 \\
SN2010ko & Ia-norm & 0.010000 & 19 & -7.10 & +15.66 & VLT & 20 & 21 & 22 \\
SN2008ar & Ia-norm & 0.026147 & 19 & -8.49 & +28.45 & Kaepora & 1 & 3 & 8 \\
SN2004as & Ia-norm & 0.031021 & 19 & -7.86 & +30.97 & Kaepora & 1 & 3 & 8 \\
SN2008bf & Ia-norm & 0.024600 & 19 & -9.15 & +31.84 & Kaepora & 1 & 3 & 23 \\
SN2005ke & Ia-91bg & 0.004880 & 19 & -8.65 & +31.26 & Kaepora,VLT & 1 & 3 & 23 \\
SN2003kf & Ia-norm & 0.007388 & 18 & -9.40 & +25.43 & Kaepora & 1 & 3 & 13 \\
SN2001eh & Ia-99aa & 0.037036 & 18 & -6.01 & +32.59 & Kaepora & 1 & 3 & 8 \\
SN2010ae & Iax & 0.003662 & 18 & -1.15 & +22.77 & WISeREP & 17 & 24 & - \\
SN2006le & Ia-norm & 0.017432 & 18 & -11.68 & +16.67 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2004eo & Ia-norm & 0.015701 & 17 & -9.99 & +30.70 & WISeREP,Kaepora,VLT & 1 & 25 & 23 \\
SN1996X & Ia-norm & 0.006945 & 17 & -3.75 & +32.89 & Kaepora & 1 & 3 & 15 \\
SN2003W & Ia-norm & 0.020071 & 17 & -11.13 & +29.97 & Kaepora & 1 & 3 & 8 \\
SN2014J & Ia-norm & 0.000677 & 17 & -8.40 & +32.12 & WISeREP & 1 & 26 & 6 \\
SN2007hj & Ia-norm & 0.014113 & 17 & -2.58 & +32.87 & Kaepora & 1 & 3 & 8 \\
SN2006N & Ia-norm & 0.014277 & 16 & -3.32 & +28.18 & Kaepora & 1 & 3 & 13 \\
SN2007ci & Ia-norm & 0.018126 & 16 & -8.05 & +27.35 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2001ay & Ia-norm & 0.030244 & 16 & -1.48 & +31.43 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2002cd & Ia-norm & 0.010344 & 16 & -8.62 & +24.02 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2007S & Ia-91T & 0.013900 & 15 & -4.69 & +32.80 & Kaepora & 1 & 3 & 23 \\
SN2006ax & Ia-norm & 0.016739 & 15 & -10.37 & +32.84 & Kaepora & 1 & 3 & 23 \\
SN2008A & Iax & 0.016428 & 15 & -7.89 & +31.54 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2003it & Ia-norm & 0.025091 & 15 & -3.24 & +31.83 & Kaepora & 1 & 3 & - \\
SN2002bf & Ia-norm & 0.024197 & 15 & +1.78 & +29.11 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1998aq & Ia-norm & 0.003699 & 15 & -9.87 & +32.88 & WISeREP,Kaepora & 1 & 3 & 15 \\
SN2006H & Ia-91bg & 0.013993 & 15 & +4.45 & +19.34 & WISeREP,Kaepora & 1 & 3 & 13 \\
SN2005bl & Ia-91bg & 0.024060 & 15 & -6.81 & +22.27 & WISeREP,Kaepora & 1 & 3 & 9 \\
SN1998es & Ia-99aa & 0.010567 & 15 & -11.36 & +29.13 & Kaepora & 1 & 3 & 8 \\
SN2012cu & Ia-norm & 0.003469 & 15 & -6.18 & +31.69 & WISeREP & 17 & 27 & - \\
SN2005el & Ia-norm & 0.014910 & 14 & -6.98 & +29.56 & Kaepora,VLT & 1 & 3 & 8 \\
SN1997do & Ia-norm & 0.010120 & 14 & -11.52 & +21.04 & Kaepora & 1 & 3 & - \\
SN2005eq & Ia-91T & 0.028977 & 14 & -8.25 & +26.61 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2002de & Ia-norm & 0.028116 & 14 & -6.09 & +26.92 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1997cn & Ia-91bg & 0.016195 & 14 & +3.84 & +28.44 & WISeREP,Kaepora & 1 & 3 & 15 \\
SN2005na & Ia-norm & 0.026322 & 14 & -1.52 & +30.60 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2005M & Ia-91T & 0.022000 & 13 & -2.74 & +30.41 & Kaepora & 1 & 3 & 23 \\
SN2007F & Ia-norm & 0.023591 & 13 & -9.52 & +32.27 & Kaepora & 1 & 3 & 6 \\
SN2000fa & Ia-norm & 0.021275 & 13 & -10.40 & +31.64 & Kaepora & 1 & 3 & 8 \\
SN2007bm & Ia-norm & 0.006211 & 13 & -11.20 & +20.54 & Kaepora & 1 & 3 & 6 \\
SN2012Z & Iax & 0.007125 & 13 & -7.55 & +22.14 & WISeREP & 17 & 28 & 6 \\
SN2000cn & Ia-norm & 0.023493 & 13 & -9.31 & +26.74 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2008Z & Ia-99aa & 0.020990 & 13 & -9.20 & +23.17 & Kaepora & 1 & 3 & 29 \\
SN1997br & Ia-91T & 0.005961 & 13 & -10.24 & +22.57 & WISeREP,Kaepora & 1 & 3 & 15 \\
SN2004gs & Ia-norm & 0.027425 & 13 & -3.45 & +31.69 & Kaepora & 1 & 3 & 9 \\
SN2003ch & Ia-norm & 0.028620 & 13 & -2.08 & +30.96 & Kaepora & 1 & 3 & 13 \\
SN1999ee & Ia-91T & 0.011415 & 13 & -9.18 & +31.35 & WISeREP,Kaepora & 1 & 30 & 31 \\
SN2007qe & Ia-norm & 0.020000 & 12 & -9.43 & +22.78 & Kaepora & 1 & 3 & 13 \\
SN2006ac & Ia-norm & 0.023106 & 12 & +6.19 & +21.73 & WISeREP,Kaepora & 1 & 3 & 13 \\
SN2004L & Ia-norm & 0.032346 & 12 & +2.42 & +32.40 & Kaepora & 1 & 3 & - \\
SN2002kf & Ia-norm & 0.019300 & 12 & +1.12 & +29.51 & Kaepora & 1 & 3 & 13 \\
SN2007al & Ia-91bg & 0.012175 & 12 & +2.38 & +16.05 & Kaepora & 1 & 3 & 23 \\
SN2010jn & Ia-norm & 0.025047 & 12 & -13.46 & +4.77 & WISeREP & 17 & 32 & - \\
SN1995al & Ia-norm & 0.005140 & 11 & +6.39 & +25.17 & Kaepora & 1 & 3 & 15 \\
SN2001cp & Ia-norm & 0.022402 & 11 & -6.80 & +28.23 & Kaepora & 1 & 3 & 8 \\
SN1998dk & Ia-norm & 0.013219 & 11 & -6.50 & +29.86 & Kaepora & 1 & 3 & - \\
SN2002jy & Ia-norm & 0.019600 & 11 & +0.12 & +30.50 & Kaepora & 1 & 3 & 13 \\
SN2004at & Ia-norm & 0.023131 & 11 & -8.56 & +29.58 & Kaepora & 1 & 3 & 8 \\
SN2004fu & Ia-norm & 0.009210 & 11 & -6.37 & +27.24 & Kaepora & 1 & 3 & - \\
SN2015bp & Ia-norm & 0.004000 & 11 & -4.81 & +32.04 & WISeREP & 17 & 33 & 22 \\
SN2007ca & Ia-norm & 0.014066 & 11 & -10.25 & +17.35 & WISeREP,Kaepora & 1 & 3 & 23 \\
SN2002eu & Ia-norm & 0.037626 & 11 & +1.10 & +27.89 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2007if & Ia-norm & 0.074200 & 11 & -9.18 & +27.99 & WISeREP,Kaepora & 1 & 3 & 23 \\
SN2001da & Ia-norm & 0.017195 & 10 & -2.01 & +10.80 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2014ek & Iax & 0.023000 & 10 & -6.25 & +24.06 & WISeREP & 17 & 34 & - \\
SN2002fk & Ia-norm & 0.007125 & 10 & -3.42 & +30.20 & Kaepora & 1 & 3 & 8 \\
SN2002cr & Ia-norm & 0.009400 & 10 & -11.20 & +24.50 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2001en & Ia-norm & 0.015871 & 10 & +1.47 & +15.01 & Kaepora & 1 & 3 & 8 \\
ASASSN-14lp & Ia-norm & 0.005100 & 10 & -11.74 & +31.81 & WISeREP,Kaepora & 1 & 35 & - \\
SN2007bc & Ia-norm & 0.020800 & 10 & -2.61 & +30.64 & WISeREP,Kaepora & 1 & 3 & 23 \\
SN1997bq & Ia-norm & 0.009346 & 10 & -10.65 & +19.08 & Kaepora & 1 & 3 & 15 \\
SN2005df & Ia-norm & 0.004316 & 10 & -9.87 & +29.94 & VLT & 17 & 36 & 37 \\
SN1998dm & Ia-norm & 0.006535 & 10 & -3.45 & +26.29 & Kaepora & 1 & 3 & 8 \\
SN1998bp & Ia-91bg & 0.010431 & 10 & -2.90 & +27.71 & Kaepora & 1 & 3 & 15 \\
SN2000dk & Ia-norm & 0.017442 & 10 & -5.12 & +28.27 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1997bp & Ia-norm & 0.008312 & 10 & -1.20 & +31.46 & Kaepora & 1 & 3 & 15 \\
SN2004ef & Ia-norm & 0.030985 & 10 & -6.27 & +31.52 & WISeREP,Kaepora,VLT & 1 & 3 & 23 \\
SN2006hb & Ia-norm & 0.015344 & 10 & +6.52 & +30.32 & Kaepora & 1 & 3 & 23 \\
SN1999gh & Ia-norm & 0.007679 & 9 & +5.49 & +28.23 & Kaepora & 1 & 3 & 15 \\
SN1998dh & Ia-norm & 0.008969 & 9 & -9.38 & +26.15 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2001N & Ia-norm & 0.021025 & 9 & +0.65 & +31.84 & Kaepora & 1 & 3 & - \\
SN2011hr & Ia-91T & 0.013279 & 9 & -7.90 & +30.59 & WISeREP & 17 & 38 & - \\
SN2002bz & Ia-norm & 0.037152 & 9 & +1.92 & +16.43 & Kaepora & 1 & 30 & - \\
SN2007fb & Ia-norm & 0.018029 & 9 & +1.71 & +32.18 & Kaepora & 1 & 3 & 6 \\
SN2002cs & Ia-norm & 0.015771 & 9 & -8.86 & +31.87 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1972E & Ia-norm & 0.001358 & 9 & +3.50 & +24.47 & WISeREP & 17 & 39 & 40,41 \\
SN2005kc & Ia-norm & 0.015120 & 9 & +6.71 & +29.34 & Kaepora & 1 & 3 & 23 \\
SN2011by & Ia-norm & 0.002843 & 9 & -11.57 & +29.32 & WISeREP,Kaepora & 1 & 26 & 22 \\
SN2006cp & Ia-norm & 0.022289 & 9 & -11.20 & +9.28 & Kaepora & 1 & 3 & 8 \\
SN2002ha & Ia-norm & 0.014400 & 9 & -4.21 & +32.23 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2001fe & Ia-norm & 0.013539 & 8 & -1.69 & +30.81 & Kaepora & 1 & 3 & 13 \\
SN2007on & Ia-norm & 0.006494 & 8 & -3.88 & +27.97 & Kaepora & 1 & 25 & 22 \\
SN2003cq & Ia-norm & 0.033283 & 8 & -5.73 & +17.44 & WISeREP,Kaepora & 1 & 3 & - \\
SN2003iv & Ia-norm & 0.034307 & 8 & -2.44 & +7.19 & Kaepora & 1 & 3 & - \\
SN1997dt & Ia-norm & 0.007318 & 8 & -10.63 & +24.04 & Kaepora & 1 & 3 & - \\
SN2006sr & Ia-norm & 0.024140 & 8 & -2.93 & +17.60 & Kaepora & 1 & 3 & 13 \\
SN2001gc & Ia-norm & 0.019290 & 8 & -8.48 & +22.00 & Kaepora & 1 & 3 & - \\
SN2002fb & Ia-91bg & 0.015567 & 8 & -4.52 & +26.82 & Kaepora & 1 & 3 & 8 \\
SN2005de & Ia-norm & 0.015184 & 8 & -9.95 & +25.75 & WISeREP,Kaepora,VLT & 1 & 30 & 8 \\
SN2007ax & Ia-91bg & 0.006878 & 8 & -2.03 & +20.95 & Kaepora & 1 & 3 & 23 \\
SN2002ck & Ia-norm & 0.029864 & 8 & -0.52 & +29.35 & Kaepora & 1 & 3 & 13 \\
SN2002dp & Ia-norm & 0.011639 & 8 & -4.77 & +22.90 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1991T & Ia-91T & 0.005791 & 8 & -12.09 & +6.80 & WISeREP,Kaepora & 1 & 30 & 42 \\
SN1999X & Ia-norm & 0.025171 & 8 & +11.98 & +28.56 & Kaepora & 1 & 3 & 15 \\
SN2002do & Ia-norm & 0.015881 & 7 & +2.00 & +30.41 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2003kc & Ia-norm & 0.033176 & 7 & -10.54 & +24.24 & Kaepora & 1 & 3 & - \\
SN1999cc & Ia-norm & 0.031328 & 7 & -3.14 & +24.94 & Kaepora & 1 & 3 & 43 \\
SN2007cq & Ia-norm & 0.026200 & 7 & -6.01 & +20.19 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN1998ab & Ia-91T & 0.027132 & 7 & -7.81 & +22.28 & Kaepora & 1 & 3 & 15 \\
SN1998co & Ia-norm & 0.018072 & 7 & -0.05 & +28.39 & Kaepora & 1 & 3 & - \\
SN2002hw & Ia-norm & 0.017535 & 7 & -6.29 & +24.40 & Kaepora & 1 & 3 & 13 \\
SN1999gp & Ia-norm & 0.026745 & 7 & -4.76 & +21.43 & Kaepora & 1 & 3 & 8 \\
SN2006gj & Ia-norm & 0.028293 & 7 & -0.65 & +19.62 & Kaepora & 1 & 3 & 9 \\
SN2008Q & Ia-norm & 0.008100 & 7 & -7.23 & +6.66 & Kaepora & 1 & 3 & 22 \\
SN2001fh & Ia-norm & 0.012990 & 7 & -3.55 & +9.16 & WISeREP,Kaepora & 1 & 3 & 13 \\
SN2001bg & Ia-norm & 0.007122 & 7 & +4.20 & +19.01 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2003hv & Ia-norm & 0.005624 & 7 & +7.86 & +25.23 & WISeREP,Kaepora,VLT & 1 & 3 & 8 \\
SN2006et & Ia-norm & 0.022639 & 7 & +2.41 & +24.68 & Kaepora & 1 & 3 & 9 \\
SN1998V & Ia-norm & 0.017586 & 7 & +0.30 & +15.03 & Kaepora & 1 & 3 & 15 \\
SN2000cp & Ia-norm & 0.034204 & 7 & -2.53 & +11.12 & WISeREP,Kaepora & 1 & 3 & - \\
SN2008ae & Iax & 0.030002 & 7 & -1.01 & +14.57 & WISeREP,Kaepora & 1 & 3 & 29 \\
SN2008hv & Ia-norm & 0.012549 & 7 & -0.94 & +11.83 & Kaepora & 1 & 25 & 9 \\
SN2005A & Ia-norm & 0.019100 & 7 & -2.21 & +32.96 & WISeREP,Kaepora & 1 & 3 & 9 \\
SN1998de & Ia-norm & 0.016471 & 7 & -6.13 & +29.31 & Kaepora & 1 & 3 & 8 \\
SN2007au & Ia-norm & 0.020584 & 7 & -5.62 & +31.60 & WISeREP,Kaepora & 1 & 3 & 13 \\
SN2007sr & Ia-norm & 0.005477 & 7 & +14.35 & +31.32 & Kaepora & 1 & 3 & 13 \\
SN2008C & Ia-norm & 0.017000 & 7 & +4.40 & +28.99 & Kaepora & 1 & 3 & 29 \\
SN1994M & Ia-norm & 0.023200 & 7 & +3.67 & +32.74 & Kaepora & 1 & 3 & 15 \\
SN2009Y & Ia-norm & 0.009353 & 7 & -5.52 & +12.37 & WISeREP,Kaepora & 1 & 25 & 23 \\
SN2004bg & Ia-norm & 0.021035 & 7 & -3.05 & +27.23 & Kaepora & 1 & 3 & 8 \\
SN2001bf & Ia-norm & 0.015501 & 6 & -0.26 & +12.48 & Kaepora & 1 & 3 & 8 \\
SN2001ck & Ia-norm & 0.034717 & 6 & +4.82 & +32.86 & Kaepora & 1 & 3 & 8 \\
SN2000dn & Ia-norm & 0.032065 & 6 & -7.66 & +16.48 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2009ag & Ia-norm & 0.008639 & 6 & -3.67 & +29.12 & WISeREP,Kaepora & 1 & 25 & - \\
SN2002jg & Ia-norm & 0.014987 & 6 & -3.46 & +25.10 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2000dg & Ia-norm & 0.038490 & 6 & -6.64 & +16.54 & Kaepora & 1 & 3 & - \\
SN1998ec & Ia-norm & 0.019900 & 6 & -3.90 & +25.49 & Kaepora & 1 & 3 & - \\
LSQ12fxd & Ia-norm & 0.032000 & 6 & -9.47 & +18.49 & WISeREP & 17 & 18 & - \\
SN1998ef & Ia-norm & 0.017742 & 6 & -8.62 & +27.83 & Kaepora & 1 & 3 & 8 \\
SN2001G & Ia-norm & 0.016770 & 6 & -5.19 & +31.16 & Kaepora & 1 & 3 & - \\
SN2004fz & Ia-norm & 0.017312 & 6 & -6.77 & +22.57 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2001ex & Ia-91bg & 0.026378 & 6 & -3.50 & +20.36 & WISeREP,Kaepora & 1 & 3 & - \\
SN2006ob & Ia-norm & 0.059239 & 6 & -6.51 & +22.87 & WISeREP,Kaepora & 1 & 25 & 9 \\
SN2004bd & Ia-norm & 0.008933 & 6 & +11.06 & +28.93 & Kaepora & 1 & 3 & 8 \\
SN2006kf & Ia-norm & 0.021301 & 6 & -8.17 & +18.15 & Kaepora & 1 & 3 & 9 \\
SN2006D & Ia-norm & 0.008600 & 6 & +2.30 & +31.24 & Kaepora & 1 & 3 & 23 \\
SN2008ha & Iax & 0.004647 & 6 & +7.46 & +23.16 & WISeREP,Kaepora & 1 & 30 & 6 \\
SN2007bd & Ia-norm & 0.030908 & 6 & -7.14 & +13.10 & Kaepora & 1 & 3 & 23 \\
SN1995bd & Ia-norm & 0.014600 & 6 & -11.99 & +20.43 & Kaepora & 1 & 3 & 15 \\
SN2005lu & Ia-norm & 0.032009 & 6 & +13.68 & +29.24 & Kaepora & 1 & 3 & 23 \\
SN2006ev & Ia-norm & 0.028733 & 6 & +5.47 & +29.60 & Kaepora & 1 & 3 & 9 \\
SN2005be & Ia-norm & 0.035000 & 6 & +7.64 & +19.23 & Kaepora & 1 & 3 & 9 \\
SN2000cf & Ia-norm & 0.036425 & 6 & +2.93 & +25.12 & Kaepora & 1 & 3 & 15,43 \\
SN2006gt & Ia-91bg & 0.044771 & 6 & +1.29 & +18.46 & Kaepora & 1 & 3 & 9 \\
SN2005cc & Iax & 0.007572 & 6 & +2.58 & +30.42 & Kaepora & 1 & 3 & 8 \\
iPTF14bdn & Ia-norm & 0.015580 & 6 & -14.59 & +20.75 & WISeREP & 17 & 44 & 22 \\
SN2004S & Ia-norm & 0.009360 & 6 & -0.00 & +16.84 & WISeREP,Kaepora & 1 & 30 & 8 \\
SN2002he & Ia-norm & 0.024564 & 6 & -8.12 & +5.59 & Kaepora & 1 & 3 & 8 \\
SN1991bg & Ia-91bg & 0.003392 & 6 & +0.14 & +29.04 & WISeREP,Kaepora & 1 & 30 & 45 \\
SN1994T & Ia-norm & 0.034656 & 5 & -0.18 & +32.70 & WISeREP,Kaepora & 1 & 3 & 15 \\
SN2007fs & Ia-norm & 0.017192 & 5 & +3.07 & +29.49 & Kaepora & 1 & 3 & 6 \\
SN1998eg & Ia-norm & 0.024760 & 5 & -0.73 & +30.51 & Kaepora & 1 & 3 & - \\
SN2007A & Ia-norm & 0.017100 & 5 & -3.42 & +13.31 & Kaepora & 1 & 3 & 23 \\
SN2008R & Ia-norm & 0.013500 & 5 & +3.19 & +27.86 & Kaepora & 1 & 3 & 9 \\
SN2001el & Ia-norm & 0.003896 & 5 & +8.47 & +28.39 & WISeREP,Kaepora,VLT & 1 & 46 & 47 \\
SN1999cp & Ia-norm & 0.009480 & 5 & -14.87 & +13.89 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2002aw & Ia-norm & 0.026145 & 5 & -1.84 & +2.10 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2010gn & Ia-norm & 0.030000 & 5 & -14.56 & -7.77 & WISeREP & 17 & 48 & 22 \\
SN1996bo & Ia-norm & 0.017285 & 5 & +3.21 & +11.08 & Kaepora & 1 & 3 & 15 \\
SN1996Z & Ia-norm & 0.007575 & 5 & +4.15 & +14.05 & Kaepora & 1 & 3 & - \\
SN1999ej & Ia-norm & 0.013723 & 5 & -1.80 & +11.02 & Kaepora & 1 & 3 & 8 \\
SN1994S & Ia-norm & 0.015177 & 5 & -3.96 & +26.48 & Kaepora & 1 & 3 & 15 \\
SN2005mz & Ia-norm & 0.017559 & 5 & -7.54 & +20.98 & Kaepora & 1 & 3 & 13 \\
SN1994Q & Ia-norm & 0.029564 & 5 & +9.97 & +12.79 & Kaepora & 1 & 3 & 15 \\
SN2008fp & Ia-norm & 0.005664 & 5 & -2.85 & +29.96 & Kaepora & 1 & 25 & 9 \\
SN1996ai & Ia-norm & 0.003156 & 5 & -0.95 & +2.16 & WISeREP,Kaepora & 1 & 3 & 15 \\
SN2002cx & Iax & 0.023963 & 5 & -4.37 & +23.99 & Kaepora & 1 & 3 & 8 \\
SN2007bj & Ia-norm & 0.016708 & 5 & +12.01 & +29.77 & WISeREP,Kaepora & 1 & 3 & 29 \\
SN2002hu & Ia-99aa & 0.030000 & 5 & -5.83 & +21.64 & Kaepora & 1 & 3 & 13 \\
SN2003ae & Ia-norm & 0.032857 & 5 & +10.68 & +31.69 & Kaepora & 1 & 30 & - \\
SN2003hx & Ia-norm & 0.007145 & 5 & +4.80 & +21.89 & Kaepora,VLT & 1 & 30 & - \\
SN2005bc & Ia-norm & 0.012272 & 5 & -6.10 & +7.77 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2003Y & Ia-91bg & 0.016942 & 5 & -6.24 & +20.95 & Kaepora & 1 & 3 & 8 \\
SN2008bc & Ia-norm & 0.015087 & 5 & -4.09 & +19.55 & Kaepora & 1 & 25 & 9 \\
SN2005bo & Ia-norm & 0.013896 & 5 & -0.09 & +26.62 & Kaepora & 1 & 3 & 8 \\
SN2001br & Ia-norm & 0.020628 & 5 & -0.45 & +26.98 & Kaepora & 1 & 3 & 8 \\
SN2001bp & Ia-norm & 0.094859 & 5 & +0.51 & +30.56 & Kaepora & 1 & 30 & - \\
SN2000dm & Ia-norm & 0.015070 & 5 & -2.85 & +25.78 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2001az & Ia-norm & 0.040695 & 5 & -3.46 & +24.74 & Kaepora & 1 & 3 & - \\
SN2006ej & Ia-norm & 0.020452 & 5 & -3.60 & +28.44 & Kaepora & 1 & 25 & 8 \\
SN1999ek & Ia-norm & 0.017522 & 5 & -0.62 & +12.15 & WISeREP,Kaepora & 1 & 3 & 49 \\
SN2008ec & Ia-norm & 0.016317 & 5 & -0.24 & +30.18 & WISeREP,Kaepora & 1 & 30 & 8 \\
SN2009aa & Ia-norm & 0.027309 & 5 & -7.75 & +9.83 & Kaepora & 1 & 25 & 23 \\
SN2000ce & Ia-norm & 0.016305 & 5 & +6.74 & +27.46 & Kaepora & 1 & 3 & 15 \\
SN2006cm & Ia-norm & 0.016341 & 5 & -1.94 & +20.67 & Kaepora & 1 & 3 & 13 \\
SN2002ef & Ia-norm & 0.023977 & 4 & -2.89 & +29.23 & WISeREP,Kaepora & 1 & 3 & - \\
SN2004br & Ia-99aa & 0.023159 & 4 & +20.05 & +26.90 & WISeREP,Kaepora & 1 & 30 & 8 \\
SN2008ei & Ia-norm & 0.037639 & 4 & +3.29 & +15.79 & WISeREP,Kaepora & 1 & 30 & - \\
SN2012hr & Ia-norm & 0.008000 & 4 & -6.82 & +14.92 & WISeREP & 17 & 50 & - \\
SN2006fw & Ia-norm & 0.083500 & 4 & -6.31 & +17.58 & WISeREP,Kaepora & 17 & 25 & - \\
SN2006py & Ia-norm & 0.057900 & 4 & -4.70 & +15.07 & WISeREP,Kaepora & 1 & 25 & - \\
SN1981B & Ia-norm & 0.006031 & 4 & -0.21 & +23.65 & WISeREP & 1 & 51 & - \\
iPTF13dge & Ia-norm & 0.015854 & 4 & -11.52 & +14.11 & WISeREP & 17 & 38 & - \\
SN2007ux & Ia-norm & 0.030915 & 4 & +4.91 & +19.48 & WISeREP,Kaepora & 1 & 3 & - \\
PTF10ops & Ia-norm & 0.060000 & 4 & -7.64 & +20.66 & WISeREP & 17 & 52 & - \\
SN1992A & Ia-norm & 0.006261 & 4 & +2.98 & +14.91 & WISeREP & 1 & 53 & - \\
SN2012cg & Ia-norm & 0.001460 & 4 & -13.28 & -5.29 & WISeREP & 1 & 54 & - \\
SN2012ht & Ia-norm & 0.003559 & 4 & -12.52 & +8.69 & WISeREP & 1 & 55 & - \\
SN2010ev & Ia-norm & 0.009200 & 4 & -1.08 & +11.79 & VLT & 1 & 46 & - \\
SN2002cf & Ia-91bg & 0.015501 & 4 & -5.42 & +16.24 & WISeREP,Kaepora & 1 & 3 & - \\
SN2002cu & Ia-norm & 0.023323 & 4 & -8.25 & +17.11 & Kaepora & 1 & 3 & - \\
SN2003D & Ia-norm & 0.022109 & 4 & +9.98 & +32.81 & Kaepora & 1 & 30 & - \\
SN2003U & Ia-norm & 0.028341 & 4 & -8.53 & -0.73 & Kaepora & 1 & 3 & - \\
SN2004ey & Ia-norm & 0.015786 & 4 & -7.09 & +31.17 & Kaepora & 1 & 25 & - \\
SN2004gc & Ia-norm & 0.032089 & 4 & +11.74 & +32.25 & Kaepora & 1 & 3 & - \\
SN2005ag & Ia-norm & 0.079665 & 4 & -0.10 & +32.22 & Kaepora & 1 & 25 & - \\
SN2005ki & Ia-norm & 0.019207 & 4 & +1.00 & +20.42 & Kaepora & 1 & 3 & - \\
SN2005mc & Ia-norm & 0.025221 & 4 & -2.18 & +25.12 & Kaepora & 1 & 3 & - \\
SN2006br & Ia-norm & 0.024590 & 4 & -0.87 & +8.00 & Kaepora & 1 & 3 & - \\
SN2006bt & Ia-norm & 0.032156 & 4 & -4.62 & +32.91 & Kaepora & 1 & 3 & 13 \\
SN2006bz & Ia-91bg & 0.027906 & 4 & -2.32 & +0.61 & Kaepora & 1 & 3 & - \\
SN2006cz & Ia-99aa & 0.041800 & 4 & -0.99 & +28.74 & Kaepora & 1 & 3 & - \\
SN2006dm & Ia-norm & 0.022019 & 4 & -7.90 & +20.44 & Kaepora & 1 & 30 & - \\
SN2006em & Ia-91bg & 0.019233 & 4 & +3.64 & +26.21 & Kaepora & 1 & 3 & - \\
SN2006gr & Ia-norm & 0.034597 & 4 & -8.89 & +24.84 & Kaepora & 1 & 3 & 8 \\
SN2006ke & Ia-91bg & 0.017182 & 4 & -0.53 & +8.38 & Kaepora & 1 & 30 & - \\
SN2006os & Ia-norm & 0.032809 & 4 & -1.08 & +26.08 & Kaepora & 1 & 25 & - \\
SN2006ot & Ia-norm & 0.053100 & 4 & -1.27 & +22.28 & Kaepora & 1 & 3 & - \\
SN2006S & Ia-99aa & 0.032102 & 4 & -3.71 & +18.68 & Kaepora & 1 & 3 & - \\
SN2008dx & Ia-91bg & 0.023026 & 4 & +2.46 & +28.84 & Kaepora & 1 & 30 & - \\
SN1995ak & Ia-norm & 0.022719 & 4 & +13.35 & +26.07 & Kaepora & 1 & 3 & - \\
SN1996bl & Ia-norm & 0.036000 & 4 & -4.06 & +18.09 & Kaepora & 1 & 3 & - \\
SN2002dl & Ia-norm & 0.016251 & 4 & -8.42 & +10.26 & Kaepora & 1 & 3 & - \\
SNF20080720-001 & Ia-norm & 0.020900 & 4 & -0.35 & +7.48 & Kaepora & 1 & 3 & - \\
SN2008ia & Ia-norm & 0.021942 & 4 & +2.88 & +15.46 & Kaepora & 1 & 25 & - \\
SN2000E & Ia-norm & 0.004750 & 4 & -7.17 & +6.77 & Kaepora & 1 & 3 & - \\
SN2002hd & Ia-norm & 0.030835 & 4 & +1.38 & +15.92 & Kaepora & 1 & 3 & - \\
SN2006bq & Ia-norm & 0.021905 & 4 & +5.33 & +13.28 & Kaepora & 1 & 3 & - \\
SN2001ic & Ia-norm & 0.044237 & 4 & +10.24 & +21.64 & Kaepora & 1 & 30 & - \\
SN2000bk & Ia-norm & 0.025444 & 4 & +11.90 & +26.52 & Kaepora & 1 & 3 & - \\
SN1997Y & Ia-norm & 0.015866 & 4 & +1.82 & +22.49 & Kaepora & 1 & 3 & - \\
SN2001E & Ia-norm & 0.019260 & 4 & +2.84 & +15.11 & Kaepora & 1 & 3 & - \\
SN1999cw & Ia-norm & 0.012372 & 4 & +13.61 & +24.46 & Kaepora & 1 & 3 & - \\
SN2006or & Ia-norm & 0.021013 & 3 & -3.91 & +4.93 & Kaepora & 1 & 30 & - \\
SN1995ac & Ia-91T & 0.050055 & 3 & -6.37 & +24.67 & Kaepora & 1 & 3 & - \\
SNF20080522-011 & Ia-norm & 0.037900 & 3 & +6.41 & +25.45 & Kaepora & 1 & 3 & - \\
SNF20080522-000 & Ia-norm & 0.045000 & 3 & +1.73 & +20.62 & Kaepora & 1 & 3 & - \\
SN2007jg & Ia-norm & 0.037131 & 3 & -4.63 & +22.64 & WISeREP,Kaepora & 1 & 3 & - \\
SN1999dk & Ia-norm & 0.014960 & 3 & -6.60 & +23.95 & Kaepora & 1 & 30 & - \\
SN1999da & Ia-91bg & 0.012695 & 3 & -2.70 & +6.17 & Kaepora & 1 & 3 & - \\
SN2006cf & Ia-norm & 0.041552 & 3 & +5.66 & +18.07 & Kaepora & 1 & 3 & - \\
SN1999cl & Ia-norm & 0.007609 & 3 & -8.25 & +25.52 & Kaepora & 1 & 3 & 8 \\
SN2006en & Ia-norm & 0.031939 & 3 & +8.55 & +30.75 & Kaepora & 1 & 30 & - \\
SN2000B & Ia-norm & 0.019827 & 3 & +8.56 & +21.48 & Kaepora & 1 & 3 & - \\
SN1993ac & Ia-norm & 0.049000 & 3 & +6.95 & +28.67 & Kaepora & 1 & 3 & - \\
SN2006eu & Ia-norm & 0.023586 & 3 & +8.08 & +16.85 & Kaepora & 1 & 3 & - \\
SN1999ef & Ia-norm & 0.039137 & 3 & +6.73 & +9.62 & Kaepora & 1 & 3 & - \\
SN1996C & Ia-norm & 0.027000 & 3 & +1.93 & +7.73 & Kaepora & 1 & 3 & - \\
SN1995D & Ia-norm & 0.006561 & 3 & +3.71 & +32.45 & Kaepora & 1 & 3 & 15 \\
SN2008hu & Ia-norm & 0.049698 & 3 & -0.59 & +20.13 & WISeREP,Kaepora & 1 & 25 & - \\
SN1995E & Ia-norm & 0.011575 & 3 & -2.85 & +31.65 & Kaepora & 1 & 3 & - \\
SN2007ba & Ia-91bg & 0.038513 & 3 & +2.93 & +5.88 & Kaepora & 1 & 3 & - \\
SN2004bk & Ia-norm & 0.023124 & 3 & +6.37 & +6.42 & WISeREP,Kaepora & 1 & 3 & - \\
SN2007N & Ia-91bg & 0.012879 & 3 & +19.77 & +32.59 & Kaepora & 1 & 25 & - \\
SN2007gi & Ia-norm & 0.004620 & 3 & -7.31 & +6.61 & Kaepora & 1 & 30 & - \\
SN2005ls & Ia-norm & 0.021118 & 3 & +10.79 & +26.49 & Kaepora & 1 & 3 & - \\
SN2007as & Ia-norm & 0.017572 & 3 & -2.68 & +26.92 & Kaepora & 1 & 25 & - \\
SN2006ef & Ia-norm & 0.017902 & 3 & +2.21 & +27.72 & WISeREP,Kaepora & 1 & 25 & - \\
SN2005bg & Ia-norm & 0.023086 & 3 & +1.96 & +8.78 & Kaepora & 1 & 25 & - \\
SN2008bq & Ia-norm & 0.034007 & 3 & +0.56 & +18.95 & Kaepora & 1 & 25 & - \\
SN2000ey & Ia-norm & 0.020407 & 3 & +7.90 & +29.30 & Kaepora & 1 & 30 & - \\
SN2006is & Ia-norm & 0.031421 & 3 & +10.14 & +13.06 & Kaepora & 17 & 25 & 23 \\
SN2003K & Ia-91T & 0.021815 & 3 & +13.43 & +20.18 & Kaepora & 1 & 30 & - \\
SN2006mr & Ia-91bg & 0.005871 & 3 & +5.58 & +11.56 & Kaepora & 1 & 25 & - \\
SN2009ig & Ia-norm & 0.008770 & 3 & -14.30 & -8.36 & WISeREP & 1 & 48 & - \\
SN2007ai & Ia-91T & 0.031662 & 3 & +1.99 & +13.56 & Kaepora & 1 & 25 & - \\
SN2002dk & Ia-91bg & 0.018533 & 3 & -3.19 & -0.16 & Kaepora & 1 & 30 & - \\
SN2002G & Ia-norm & 0.033737 & 3 & -4.42 & +16.89 & Kaepora & 1 & 3 & - \\
SN2003gn & Ia-norm & 0.034450 & 3 & -5.00 & +3.65 & Kaepora & 1 & 3 & - \\
SN2009ad & Ia-norm & 0.028400 & 3 & -0.50 & +32.53 & Kaepora & 1 & 25 & - \\
SN2009D & Ia-norm & 0.025007 & 3 & -4.10 & +29.07 & WISeREP & 17 & 25 & - \\
SN1997cw & Ia-norm & 0.017100 & 2 & +12.15 & +32.79 & Kaepora & 1 & 30 & - \\
LSQ12gpw & Ia-norm & 0.058000 & 2 & -1.09 & -1.09 & WISeREP & 17 & 56 & - \\
SN2008bt & Ia-91bg & 0.015364 & 2 & -1.08 & +10.97 & Kaepora & 1 & 30 & - \\
SN2017cbv & Ia-norm & 0.003990 & 2 & -11.60 & -0.55 & WISeREP & 1 & 57 & - \\
SN2008gp & Ia-norm & 0.033413 & 2 & +15.39 & +15.61 & WISeREP,Kaepora & 1 & 25 & - \\
SN2009ab & Ia-norm & 0.011171 & 2 & +2.72 & +4.71 & Kaepora & 1 & 25 & - \\
SN2007nq & Ia-norm & 0.045031 & 2 & +11.08 & +16.83 & Kaepora & 1 & 3 & - \\
SN1989M & Ia-norm & 0.005060 & 2 & +2.49 & +3.48 & Kaepora & 1 & 30 & - \\
SN2008gl & Ia-norm & 0.034017 & 2 & -1.48 & +26.60 & Kaepora & 1 & 25 & - \\
SN1999gd & Ia-norm & 0.018509 & 2 & +1.10 & +7.91 & Kaepora & 1 & 3 & - \\
SN2005al & Ia-norm & 0.012402 & 2 & +14.73 & +18.63 & Kaepora & 1 & 25 & - \\
SN2004bw & Ia-norm & 0.021198 & 2 & +6.59 & +6.59 & WISeREP,Kaepora & 1 & 30 & - \\
SN2007ap & Ia-norm & 0.015818 & 2 & +7.43 & +11.38 & Kaepora & 1 & 3 & - \\
SN2006oa & Ia-norm & 0.060000 & 2 & -10.57 & -4.91 & WISeREP & 1 & 3 & - \\
SN2006eq & Ia-norm & 0.049509 & 2 & +26.42 & +27.38 & Kaepora & 1 & 3 & - \\
SN2007gk & Ia-norm & 0.026632 & 2 & -1.72 & +19.65 & Kaepora & 1 & 30 & - \\
SN2005eu & Ia-norm & 0.034900 & 2 & -8.77 & -5.17 & WISeREP,Kaepora & 1 & 3 & 8 \\
SN2007fr & Ia-norm & 0.050899 & 2 & -5.83 & -1.25 & Kaepora & 1 & 30 & - \\
SN2007cs & Ia-norm & 0.017559 & 2 & +12.15 & +24.81 & Kaepora & 1 & 30 & - \\
SN2004gu & Ia-norm & 0.045859 & 2 & -6.08 & -4.37 & Kaepora & 1 & 25 & - \\
SN2001cj & Ia-norm & 0.024233 & 2 & +13.63 & +23.43 & Kaepora & 1 & 3 & - \\
SN2003he & Ia-norm & 0.025504 & 2 & +2.71 & +8.54 & Kaepora & 1 & 30 & - \\
SN2003gt & Ia-norm & 0.015657 & 2 & -5.07 & +17.61 & Kaepora & 1 & 30 & - \\
SN2003gq & Iax & 0.021448 & 2 & -0.59 & +1.46 & Kaepora & 1 & 3 & - \\
SN2015F & Ia-norm & 0.004890 & 2 & -14.37 & -2.78 & WISeREP,Kaepora & 1 & 58 & - \\
SN2004go & Ia-norm & 0.029170 & 2 & +16.13 & +26.08 & WISeREP,Kaepora & 1 & 30 & - \\
SN2003ai & Ia-norm & 0.036177 & 2 & -9.74 & +7.24 & Kaepora & 1 & 30 & - \\
SN2002et & Ia-norm & 0.027576 & 2 & +11.92 & +14.89 & Kaepora & 1 & 30 & - \\
SN2002el & Ia-norm & 0.028460 & 2 & +11.82 & +21.49 & Kaepora & 1 & 30 & - \\
SN2002eb & Ia-norm & 0.027536 & 2 & +1.68 & +26.08 & Kaepora & 1 & 30 & - \\
SN2008dt & Ia-norm & 0.035391 & 2 & +9.27 & +9.27 & WISeREP,Kaepora & 1 & 30 & - \\
SN2002df & Ia-norm & 0.028680 & 2 & +2.69 & +6.55 & Kaepora & 1 & 30 & - \\
SN2002db & Ia-norm & 0.036222 & 2 & +2.40 & +9.21 & Kaepora & 1 & 30 & - \\
SN2002cv & Ia-norm & 0.004240 & 2 & -1.40 & +18.53 & Kaepora & 1 & 30 & - \\
SN2000cw & Ia-norm & 0.030100 & 2 & +3.46 & +5.30 & Kaepora & 1 & 3 & - \\
SN2005ao & Ia-norm & 0.038407 & 2 & -1.29 & +0.52 & Kaepora & 1 & 30 & - \\
SN2005er & Ia-91bg & 0.026175 & 2 & +1.67 & +5.64 & Kaepora & 1 & 30 & - \\
SN2006je & Ia-norm & 0.037996 & 2 & +20.18 & +26.02 & Kaepora & 1 & 30 & - \\
SN2007bz & Ia-norm & 0.021778 & 2 & +1.49 & +17.04 & Kaepora & 1 & 3 & - \\
SN2006te & Ia-norm & 0.031592 & 2 & +23.84 & +28.62 & Kaepora & 1 & 3 & - \\
SN1997E & Ia-norm & 0.013539 & 2 & +19.96 & +20.00 & Kaepora & 1 & 3 & - \\
SN1991M & Ia-norm & 0.007235 & 2 & +2.17 & +27.00 & WISeREP & 1 & 30 & - \\
SN2001L & Ia-norm & 0.015461 & 2 & +9.22 & +21.57 & Kaepora & 1 & 30 & - \\
SN1998dx & Ia-norm & 0.054224 & 2 & +5.05 & +27.77 & Kaepora & 1 & 3 & - \\
SN1999bh & Ia-norm & 0.017205 & 2 & +5.08 & +19.91 & Kaepora & 1 & 3 & - \\
SN2000cu & Ia-norm & 0.020324 & 2 & +7.31 & +9.35 & Kaepora & 1 & 3 & - \\
SN2005dv & Ia-norm & 0.010404 & 2 & -2.72 & -0.57 & WISeREP,Kaepora & 1 & 30 & - \\
SN1992G & Ia-norm & 0.005290 & 2 & +18.09 & +23.41 & WISeREP,Kaepora & 1 & 30 & - \\
SN2006cs & Ia-91bg & 0.023676 & 2 & +2.21 & +2.28 & Kaepora & 1 & 30 & - \\
SN2006bw & Ia-norm & 0.030002 & 2 & +7.82 & +30.18 & Kaepora & 1 & 3 & - \\
SN2005W & Ia-norm & 0.008889 & 2 & +24.64 & +28.66 & Kaepora & 1 & 25 & - \\
SN2005ms & Ia-norm & 0.025204 & 2 & -1.88 & +14.62 & Kaepora & 1 & 30 & - \\
SN2005dm & Ia-91bg & 0.016838 & 2 & +5.23 & +5.23 & WISeREP,Kaepora & 1 & 30 & - \\
\end{tabular}
\end{table}

